QERA: an Analytical Framework for Quantization Error Reconstruction

The growing number of parameters and computational demands of large language models (LLMs) present significant challenges for their efficient deployment. Recently, there is an increasing interest in quantizing weights to extremely low precision while offsetting the resulting error with low-rank, high-precision error reconstruction terms. The combination of quantization and low-rank approximation is now popular in both adapter-based, parameter-efficient fine-tuning methods such as LoftQ and low-precision inference techniques including ZeroQuant-V2. Usually, the low-rank terms are calculated via the singular value decomposition (SVD) of the weight quantization error, minimizing the Frobenius and spectral norms of the weight approximation error. Recent methods like LQ-LoRA and LQER introduced hand-crafted heuristics to minimize errors in layer outputs (activations) rather than weights, resulting improved quantization results. However, these heuristic methods lack an analytical solution to guide the design of quantization error reconstruction terms. In this paper, we revisit this problem and formulate an analytical framework, named Quantization Error Reconstruction Analysis (QERA), and offer a closed-form solution to the problem. We show QERA benefits both existing low-precision fine-tuning and inference methods -- QERA achieves a fine-tuned accuracy gain of $\Delta_{\text{acc}}$ = 6.05% of 2-bit RoBERTa-base on GLUE compared to LoftQ; and obtains $\Delta_{\text{acc}}$ = 2.97% higher post-training quantization accuracy of 4-bit Llama-3.1-70B on average than ZeroQuant-V2 and $\Delta_{\text{ppl}}$ = - 0.28 lower perplexity on WikiText2 than LQER.

==> figures/fig_roberta-mrpc-convergence-3bit.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/raw/roberta_mrpc_convergence_3bit.pdf}
    \caption{Faster convergence of \loqerdiag{} on MRPC.}
    \label{fig:roberta-mrpc-convergence-3bit}
\end{figure}

==> figures/fig_runtime-vs-moel-size.tex <==
%\begin{figure}
\begin{wrapfigure}{R}{0.40\textwidth}
    \ifdefined\isiclr
        \vspace{-2em}
    \fi
    \centering
    \includegraphics[width=0.38\textwidth]{figures/raw/vis_runtime.pdf}
    \ifdefined\isiclr
        \vspace{-1em}
    \fi
    \caption{\loqer{} quantization time \textit{vs.} model sizes.
        ``A'' and ``E'' denote \loqerdiag{} and \loqerrxx{} respectively. \loqerrxx{} is slower for computing matrix square root on CPUs.}
    \ifdefined\isiclr
        \vspace{-1em}
    \fi
    \label{fig:runtime-vs-model-size}
\end{wrapfigure}
%\end{figure}


==> figures/fig_sqrtm-error-vs-hidden-size.tex <==
%\begin{figure}[ht]
    \begin{wrapfigure}{R}{0.4\textwidth}
    %\vspace{-2em}
    \centering
    \includegraphics[width=0.38\textwidth]{figures/raw/sqrtm_error_vs_rxx_size.pdf}
    \caption{
        Estimated error ratio of the square root of the auto-correlation matrix calculated by the blocked algorithm with different hidden sizes.
        %The error ratio is calculated as $\frac{\|error\|}{\|R_{xx}\|}$.
        The error ratio increases as the model is larger. This can be one reason for the less PTQ improvement of
        \loqerrxx{} compared to \loqerdiag{} on larger models, besides that a larger LLM is more resistant to quantization.
    }
    %\vspace{-2em}
    \label{fig:sqrtm-error-vs-hidden-size}
    \end{wrapfigure}
%\end{figure}

==> figures/tab_llm_ptq_other_baselines.tex <==
\begin{wraptable}{r}{0.5\textwidth}
    %\begin{table}[]
    \ifdefined\isiclr
        \vspace{-1em}
    \fi
    \caption{Perplexity ($\downarrow$) on WikiText2 compared to QuiP\#, a leading 2-bit PTQ method that does not use quantization error reconstruction.}
    \ifdefined\isiclr
        \vspace{-1em}
    \fi
    \begin{center}
        \begin{small}
            \begin{tabular}{@{}lcccc@{}}
                \toprule
                Methods     & Gemma-2 & \multicolumn{2}{c}{LLaMA-2} & LLaMA-3      \\ \cmidrule(l){2-5}
                            & 2B      & 7B                          & 13B     & 8B \\ \midrule
                BF16        &         &                             &         &    \\
                QuiP\#      &         &                             &         &    \\
                \loqerrxx{} &         &                             &         &    \\ \bottomrule
            \end{tabular}
        \end{small}
    \end{center}
    \ifdefined\isiclr
        \vspace{-2em}
    \fi
    \label{tab:llm-ptq-other-baselines}
    %\end{table}
\end{wraptable}

==> figures/tab_old_llama-2_experiments.tex <==
\begin{table}[]
    \color{blue}
    \caption{QPEFT experiments of \llama{}-2 on WikiText2 matching LoftQ setup. QERA-approx outperforms LoftQ.}
    \centering
    \begin{small}
        \begin{tabular}{@{}cccccc@{}}
            \toprule
            Method      & W-bits & \multicolumn{2}{c}{Llama-2-7B} & \multicolumn{2}{c}{Llama-2-13B}                                                \\ \cmidrule(l){3-6}
                        &        & WikiText ($\downarrow$)        & GSM8K ($\uparrow$)              & WikiText ($\downarrow$) & GSM8K ($\uparrow$) \\ \midrule
            LoRA        & 16     & 5.02                           & 39.4                            & 5.09                    & 46.4               \\ \midrule
            LoftQ       & 4.25   & 5.26                           & 34.7                            & 5.14                    & 44.8               \\
            QERA-approx & 4.25   & \textbf{5.11}                  & \textbf{35.8}                   & \textbf{5.12}           & \textbf{45.1}      \\ \bottomrule
        \end{tabular}
    \end{small}
    \label{tab:appendix:qpeft-old-llama-2}
\end{table}

==> figures/tab_qera-vs-lq-lora-ptq.tex <==
\begin{table}[]
    \color{blue}
    \caption{Comparison of QERA-exact and LQ-LoRA on WikiText2 via PTQ experiments.
        QERA-exact achieves lower perplexity most of the time.}
    \centering
    \begin{small}
        \begin{tabular}{@{}llcccc@{}}
            \toprule
            \multirow{2}{*}{W-bits} & \multirow{2}{*}{Method} & TinyLlama      & Gemma-2        & Phi-3.5        & LLaMA-3.1      \\ \cmidrule(l){3-6}
                                    &                         & 1.1B           & 2B             & 3.8B           & 8B             \\ \midrule
            16                      & BF16                    & 13.98          & 13.08          & 11.50          & 7.55           \\ \midrule
            \multirow{2}{*}{4.25}   & LQ-LoRA                 & \textbf{15.98} & 14.76          & 13.43          & 8.64           \\
                                    & QERA-exact              & 16.16          & \textbf{14.12} & \textbf{12.30} & \textbf{8.33}  \\ \midrule
            \multirow{2}{*}{3.25}   & LQ-LoRA                 & 20.38          & 21.53          & \textbf{19.15} & 11.77          \\
                                    & QERA-exact              & \textbf{19.51} & \textbf{19.97} & 20.37          & \textbf{11.39} \\ \bottomrule
        \end{tabular}
    \end{small}
    \label{tab:appendix:qera-vs-lq-lora-ptq}
\end{table}

==> figures/tab_qera-vs-lq-lora-qpeft.tex <==
\begin{table}[]
    \color{blue}
    \caption{Comparison of QERA-approx and LQ-LoRA on LLaMA-2-7B and LLaMA-3.1-8B via QPEFT experiments. QERA-approx consistently outperforms LQ-LoRA.}
    \centering
    \begin{small}
        \begin{tabular}{@{}llcccc@{}}
            \toprule
            \multirow{2}{*}{W-bits} & \multirow{2}{*}{Method} & \multicolumn{2}{c}{LLaMA-2-7B} & \multicolumn{2}{c}{LLaMA-3.1-8B}                                   \\ \cmidrule(l){3-6}
                                    &                         & SlimPajama                     & GSM8K                            & SlimPajama     & GSM8K          \\ \midrule
            16                      & LoRA                    & 6.17                           & 39.40                            & 8.07           & 55.72          \\ \midrule
            \multirow{2}{*}{4.25}   & LQ-LoRA                 & 6.36                           & 31.12                            & 8.71           & 54.67          \\
                                    & QERA-approx             & \textbf{6.33}                  & \textbf{32.26}                   & \textbf{8.68}  & \textbf{55.24} \\ \midrule
            \multirow{2}{*}{2.25}   & LQ-LoRA                 & 11.49                          & 18.63                            & 22.14          & 17.84          \\
                                    & QERA-approx             & \textbf{10.56}                 & \textbf{18.78}                   & \textbf{20.07} & \textbf{19.41} \\ \bottomrule
        \end{tabular}
    \end{small}
    \label{tab:appendix:qera-vs-lq-lora-qpeft}
\end{table}

==> figures/tab_qpeft_2.125-bit_glue.tex <==
\begin{table}[]
    \color{blue}
    \caption{QPEFT experiments of 2.125-bit RoBERTA-base on GLUE mathcing LoftQ setup. QERA-approx still outperforms LoftQ though both fine-tuned models have poor performance.}
    \centering
    \begin{small}
        \begin{tabular}{@{}lccccccccc@{}}
            \toprule
            Method      & W-bits                 & MNLI           & QNLI           & RTE   & SST            & CoLA & QQP            & STSB           & Avg. $^*$      \\ \midrule
            LoftQ       & \multirow{2}{*}{2.125} & 74.81          & 82.57          & 55.96 & 85.09          & 0    & 85.62          & 52.46          & 71.26          \\
            QERA-approx &                        & \textbf{80.26} & \textbf{85.72} & 55.96 & \textbf{89.11} & 0    & \textbf{87.34} & \textbf{66.68} & \textbf{77.51} \\ \bottomrule
        \end{tabular}
    \end{small}
    \label{tab:appendix:qpeft-2.125-bit-glue}
\end{table}

==> figures/tab_runtime_qera-approx-vs-loftq.tex <==
\begin{table}[]
    \color{blue}
    \caption{Runtime comparison of \loftq{} (5-iter) and \loqerdiag{} across various model sizes.
        For \loftq{} the runtime denotes the quantization time,
        while for \loqerdiag{} it denotes the calibration time plus the quantization time.
        \loqerdiag{} is faster than \loftq{} by 2-4 times. \tbgreen{@Reviwer 8w8V}}
    \centering
    \begin{small}
        \begin{tabular}{@{}lccccc@{}} \toprule
            Method      & 1B          & 3B           & 7B           & 13B          & 30B          \\ \midrule
            LoftQ       & 170s        & 1037s        & 3068s        & 7084s        & 45361s       \\
            QERA-approx & 70s         & 264s         & 738s         & 1952s        & 12495s       \\
            Speed up    & 2.4$\times$ & 3.94$\times$ & 4.16$\times$ & 3.63$\times$ & 3.62$\times$ \\ \bottomrule
        \end{tabular}
    \end{small}
    \label{tab:appendix:runtime-qera-approx-vs-loftq}
\end{table}

==> figures/tab_space_complexity_loftq.tex <==
\begin{table}[]
    \color{blue}
    \caption{Memory complexity of \loqerdiag{} of a linear layer. $(m,n)$ are the input and output feature sizes,
        $k$ denotes the rank.}
    \centering
    \begin{footnotesize}
        \begin{tabular}{@{}lll@{}}
            \toprule
            Phase                         & Operation                       & Complexity \\ \midrule
            \multirow{4}{*}{Quantization} & Full-precision weight matrix    & $O(mn)$    \\
                                          & Quantized weight matrix         & $O(mn)$    \\
                                          & SVD on the scaled weight matrix & $O(mn)$    \\
                                          & Low-rank terms                  & $O(mk+nk)$ \\ \bottomrule
        \end{tabular}
    \end{footnotesize}
    \label{tab:appendix:space-complexity-loftq}
\end{table}

==> figures/tab_space_complexity_qera-approx.tex <==
\begin{table}[h]
    \color{blue}
    \caption{Memory complexity of \loqerdiag{} of a linear layer. $(m,n)$ are the input and output feature sizes,
        $k$ denotes the rank, and $b$ is the number of calibration samples.}
    \centering
    \begin{small}
        \begin{tabular}{@{}lll@{}}
            \toprule
            Phase                         & Operation                       & Complexity    \\ \midrule
            \multirow{2}{*}{Calibration}  & GEMM of linear forward pass     & $O(bm+mn+bn)$ \\
                                          & Partial sum of $\mS$            & $O(m)$        \\ \midrule
            \multirow{5}{*}{Quantization} & Full-precision weight matrix    & $O(mn)$       \\
                                          & Quantized weight matrix         & $O(mn)$       \\
                                          & SVD on the scaled weight matrix & $O(mn)$       \\
                                          & Inverse of $\mS$                & $O(m)$        \\
                                          & Low-rank terms                  & $O(mk+nk)$    \\ \bottomrule
        \end{tabular}
    \end{small}
    \label{tab:appendix:space-complexity-qera-approx}
\end{table}

==> figures/tab_space_complexity_qera-exact.tex <==
\begin{table}[h]
    \color{blue}
    \caption{Memory complexity of \loqerrxx{} of a linear layer. $(m,n)$ are the input and output feature sizes,
        $k$ denotes the rank, and $b$ is the number of calibration samples.}
    \centering
    \begin{footnotesize}
        \begin{tabular}{@{}lll@{}}
            \toprule
            Phase                         & Operation                                       & Complexity    \\ \midrule
            \multirow{2}{*}{Calibration}  & GEMM of linear forward pass                     & $O(bm+mn+bn)$ \\
                                          & Partial sum of $\mR_{\sX\sX}$                   & $O(m^2)$      \\ \midrule
            \multirow{6}{*}{Quantization} & Full-precision weight matrix                    & $O(mn)$       \\
                                          & Quantized weight matrix                         & $O(mn)$       \\
                                          & SVD on the scaled weight matrix                 & $O(mn)$       \\
                                          & Matrix square root of $\mR_{\sX\sX}$            & $O(m^2)$      \\
                                          & Matrix Inverse of $({\mR_{\sX\sX}}^{1/2})^{-1}$ & $O(m^2)$      \\
                                          & Low-rank terms                                  & $O(mk+nk)$    \\ \bottomrule
        \end{tabular}
    \end{footnotesize}
    \label{tab:appendix:space-complexity-qera-exact}
\end{table}

==> figures/tab_time_complexity_loftq.tex <==
\begin{table}[h]
    \color{blue}
    \caption{Computational complexity of \loftq{}. $(m,n)$ are the input and output feature sizes,
        $k$ denotes the rank, and $t$ is the iteration number.}
    \centering
    \begin{footnotesize}
        \begin{tabular}{@{}ll@{}}
            \toprule
            Operation               & Complexity              \\ \midrule
            Update quantized weight & $O(tmnk)$               \\
            Residual subtraction    & $O(tmn)$                \\
            SVD on weight matrix    & $O(tmn\cdot\min(m, n))$ \\ \bottomrule
        \end{tabular}
    \end{footnotesize}
    \label{tab:appendix:time-complexity-qera-loftq}
\end{table}

==> figures/tab_time_complexity_qera-approx.tex <==
\begin{table}[h]
    \color{blue}
    \caption{Computational complexity of \loqerdiag{}. $(m,n)$ are the input and output feature sizes,
        $k$ denotes the rank, and $b$ is the number of calibration samples.}
    \centering
    \begin{footnotesize}
        \begin{tabular}{@{}ll@{}}
            \toprule
            Operation               & Complexity             \\ \midrule
            Scale matrix $\mS$      & $O(m^2\log_2 m)$       \\
            SVD on weight matrix    & $O(mn\cdot\min(m, n))$ \\
            Product to form $\mC_k$ & $O(m^3)$               \\ \bottomrule
        \end{tabular}
    \end{footnotesize}
    \label{tab:appendix:time-complexity-qera-approx}
\end{table}

==> figures/tab_time_complexity_qera-exact.tex <==
\begin{table}[h]
    \color{blue}
    \caption{Computational complexity of \loqerrxx{} of a linear layer. $(m,n)$ are the input and output feature sizes,
        $k$ denotes the rank, and $b$ is the number of calibration samples.}
    \centering
    \begin{footnotesize}
        \begin{tabular}{@{}ll@{}}
            \toprule
            Operation                              & Complexity             \\ \midrule
            Auto-correlation matrix $\mR_{\sX\sX}$ & $O(bm^2)$              \\
            Matrix square root of $\mR_{\sX\sX}$   & $O(m^3)$               \\
            Inverse of $\mR_{\sX\sX}^\frac{1}{2}$  & $O(m^3)$               \\
            SVD on weight matrix                   & $O(mn\cdot\min(m, n))$ \\
            Product to form $\mC_k$                & $O(m^3)$               \\
            \bottomrule
        \end{tabular}
    \end{footnotesize}
    \label{tab:appendix:time-complexity-qera-exact}
\end{table}
